Zero-rating of Content and its Effect on the Quality of Service in the Internet

The ongoing net neutrality debate has generated a lot of heated discussions on whether or not monetary interactions should be regulated between content and access providers. Among the several topics discussed, `differential pricing' has recently received attention due to `zero-rating' platforms proposed by some service providers. In the differential pricing scheme, Internet Service Providers (ISPs) can exempt data access charges for on content from certain CPs (zero-rated) while no exemption is on content from other CPs. This allows the possibility for Content Providers (CPs) to make `sponsorship' agreements to zero-rate their content and attract more user traffic. In this paper, we study the effect of differential pricing on various players in the Internet. We first consider a model with a monopolistic ISP and multiple CPs where users select CPs based on the quality of service (QoS) and data access charges. We show that in a differential pricing regime 1) a CP offering low QoS can make have higher surplus than a CP offering better QoS through sponsorships. 2) Overall QoS (mean delay) for end users can degrade under differential pricing schemes. In the oligopolistic market with multiple ISPs, users tend to select the ISP with lowest ISP resulting in same type of conclusions as in the monopolistic market. We then study how differential pricing effects the revenue of ISPs.

==> CPGame1.tex <==
For ease of notation, we attach subscripts $00, 11, 01,$ and $10$ to the minimum equilibrium utility $\alpha$ to denote the cases where action of CPs are $(S,S), (N,N), (S,N),$ and $(N,S)$, respectively. The equilibrium rates for these actions profiles can be directly obtained from Lemma \ref{lma:EquRates}.

\begin{thm}
	\label{thm:EquRatesSpecialCases}
	The equilibrium arrival rates when each CP either plays either S or N are as follows:
	\begin{enumerate}
		\item When the actions are $(0,0)$:
                     \\ $\tilde{\lambda_i^*}=m_i+\lambda_0-\frac{1}{\alpha_{00}}$ for $ i=1,2,$ where $ \alpha_{00}=\frac{2}{\overline{m}}$  and $\overline{m}=m_1+m_2-\lambda.$ Further,  $RGF=1+\frac{2\lambda_0}{\lambda}$.
		\item When the actions are $(1,1)$:
		\\$\tilde{\lambda_i^*}=m_i-\frac{1}{\alpha_{11}-c} \;\; \mbox{for} \;\; i=1,2;  \;\; \alpha_{11}=c+\frac{2}{\overline{m}}$  where  $\overline{m}=m_1+m_2-\lambda.$ There is no gain for ISP and $RGF=1$
		\item When the actions are $(0,1)$:
		\\$\tilde{\lambda_1^*}=m_1+\lambda_0-\frac{1}{\alpha_{01}}$ and
		$\tilde{\lambda_2^*}=m_2-\frac{1}{\alpha_{01}-c}$ where $\alpha_{01}=c/2+1/\overline{m}+\sqrt{c^2/4+ 1/\overline{m}^2}$
		and can be bounded as
		\begin{equation}
		\label{eqn:DelayBounds}
		c+ 1/\overline{m} \leq \alpha_{01}\leq c+ 2/\overline{m}.
		\end{equation}
        where $\overline{m}=m_1+m_2-\lambda$. RGF for ISP is $1+\frac{\lambda_0}{\lambda}$
		\item When the actions are $(1,0)$:
		\\$\tilde{\lambda_i^*}=m_1-\frac{1}{\alpha_{10}-c}$ and $\tilde{\lambda_2^*}=m_2+\lambda_0-\frac{1}{\alpha_{10}} $ where  $\overline{m}=m_1+m_2-\lambda $ and $\alpha_{10}=\alpha_{01}$. The RGF for the ISP is $RGF=1+\frac{\lambda_0}{\lambda}.$%\hfill\IEEEQED
	\end{enumerate}
\end{thm}

\begin{cor}
	\label{corol:MinCostRelations}
	We have $\alpha_{00}=\alpha_{11}-c$ and $\alpha_{01}\geq \alpha_{00}\geq \alpha_{10}-c$.
\end{cor}

With each CP playing two actions $\{\textit{S,N}\}$ we have $2\times 2$ matrix games between the CPs. The utilities for both CPs over actions $\{\textit{S,N}\}$ are given in Table 1. 
%\begin{table}
%	\begin{center}
%		\begin{tabular}{|c|c|c|}\hline
%			$ A $ & $S $ & $ N $ \\ \hline
%			S & $U_1=(\beta-\rho c)(m_1-\lambda_0-1/\alpha_{00})$ & $U_1=(\beta-\rho c)(m_1-\lambda_0-1/\alpha_{01})%$ \\
%			$ $ & $U_2=(\beta-\rho c)(m_2-\lambda_0-1/\alpha_{00})$ & $U_2=\beta(m_2-\lambda_0-1/(\alpha_{01}-c))$ \%\ \hline
%			N & $U_1=\beta(m_1-\lambda_0-1/(\alpha_{10}-c))$ & $U_1=\beta(m_1-\lambda_0-1/(\alpha_{11}-c))$ \\
%			$ $ & $U_2=(\beta-\rho c)(m_2-\lambda_0-1/\alpha_{10})$ & $U_2=\beta(m_2-\lambda_0-1/(\alpha_{11}-c))$ \%\ \hline
%		\end{tabular}
%	\end{center}
%	\caption{Utility for CPs over actions $\{S,N\}$}  \label{tab:Utilities}
%\end{table}

\begin{table}
	\begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $S $ \\ \hline
			S & $U_1=(\beta-\rho c)(m_1+\lambda_0-1/\alpha_{00})$ \\
			$ $ & $U_2=(\beta-\rho c)(m_2+\lambda_0-1/\alpha_{00})$ \\ \hline
			N & $U_1=\beta(m_1+\lambda_0-1/(\alpha_{10}-c))$ \\
			$ $ & $U_2=(\beta-\rho c)(m_2+\lambda_0-1/\alpha_{10})$\\ \hline
		\end{tabular}
	\end{center}
    \begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ &$ N $ \\ \hline
			S & $U_1=(\beta-\rho c)(m_1+\lambda_0-1/\alpha_{01})$ \\
			$ $ & $U_2=\beta(m_2+\lambda_0-1/(\alpha_{01}-c))$ \\ \hline
			N & $U_1=\beta(m_1+\lambda_0-1/(\alpha_{11}-c))$ \\
			$ $ & $U_2=\beta(m_2+\lambda_0-1/(\alpha_{11}-c))$ \\ \hline
		\end{tabular}
	\end{center}
	\caption{Utility for CPs over actions $\{S,N\}$}  \label{tab:Utilities}
\end{table}

The following theorem states the conditions for the existence of PNE. 
\begin{thm}
	\label{thm:PNE}
Let $\rho, c, \beta$ be given. Then,
\begin{itemize}
	\item $(S,S)$ is a PNE if and only if  
	\begin{equation}
	\label{eqn:SS}
	\rho/\beta\leq A:=\frac{ 1/(\alpha_{10}-c)+\lambda_0-1/\alpha_{00}}{c(m_2+\lambda_0-1/\alpha_{00})}
	\end{equation}
	\item $(N,N)$ is a PNE if and only if 
	\begin{equation}
		\label{eqn:NN}
\rho/\beta \geq B:=\frac{1/(\alpha_{11}-c)+\lambda_0-1/\alpha_{01}}{c(m_1+\lambda_0-1/\alpha_{01})}
	\end{equation}
	\item $(S,N)$ is a PNE if and only if
	\begin{equation}
		\label{eqn:SN}
	\frac{ 1/(\alpha_{10}-c)+\lambda_0-1/\alpha_{00}}{c(m_2+\lambda_0-1/\alpha_{00})} \leq \rho/\beta \leq	\frac{1/(\alpha_{11}-c)+\lambda_0-1/\alpha_{01}}{c(m_1+\lambda_0-1/\alpha_{01})}
	\end{equation}
	\item $(N,S)$ is a PNE if and only if
	\begin{eqnarray}
		\label{eqn:NS}
C:=\frac{ 1/(\alpha_{10}-c)+\lambda_0-1/\alpha_{00}}{c(m_1+\lambda_0-1/\alpha_{00})} \leq \rho/\beta  \nonumber\\
\rho/\beta  \leq \frac{1/(\alpha_{11}-c)+\lambda_0-1/\alpha_{01}}{c(m_2+\lambda_0-1/\alpha_{01})}=:D.
	\end{eqnarray}
\end{itemize}
\end{thm}

\begin{cor}
	\label{corol:NoPNE}
	For all $c>0$, we have $C>D$ and hence $(N,S)$ cannot be a PNE.
\end{cor}
Theorem \ref{thm:PNE} gives a characterization of the PNE and Figure \ref{fig:PNE1} depicts the range of $\rho/\beta$ for different PNE.

%\begin{figure*}[!h]
%	\centering
%		\subfloat[]{\includegraphics[scale=0.05]{figures/AB1}%
%		\label{fig:AB1}}
%	\hspace{0.6cm}
%	\subfloat[]{\includegraphics[scale=0.05]{figures/AB2}%
%		\label{fig:AB2}}
%		\caption {The comparision $A$ and $B$ with respect to change in parameters $c$ in Figs. \ref{fig:AB1} and \ref{fig:AB2} for different values of $m_1$.   We set $\beta=1$,$\rho=.9$, $\lambda=1200$, $\lambda_0=200$ and $m_2=1000$ throughout. In Fig. \ref{fig:AB1}, we set $m_1=900$ and in Fig. \ref{fig:AB2}, we set $m_1=650$.}
%	\label{fig:Gain}
%\end{figure*}

\begin{figure}[!h]
	\centering
	\includegraphics[scale=.245]{figures/PNE1}
	\caption{The PNE as a function of $\rho/\beta$.}
		\label{fig:PNE1}
\end{figure}

We study the behaviour of RGF and the shift in PNE point with respect to system parameters $\lambda,$ $\lambda_0$ and $c$ .  From Fig. \ref{fig:Gain1} it is observed that as $\lambda$ increases, RGF initially decreases steeply and then at a slower rate. This change is due to shift of PNE point from \{S,S\} to \{S,N\}. This shift of PNE point has been caused by the change in the values of A and B with the increase in $\lambda$. It is inferred that when CPS offer the subsidy, the gain for ISP decreases with increase in usual traffic flow, keeping exogenous traffic to be fixed.  Fig. \ref{fig:Gain2} shows that RGF initially increases at smaller rate with increase in exogenous traffic ($\lambda_0$) and later the rate increases. This shift in behaviour is again due to shifting PNE points from \{S,N\} to \{S,S\} as CPs are likely to go for full sponsorship if more exogenous traffic is generated. Thus, ISP is benefitted when higher exogenous traffic is generated as more revenue is generated. While Fig. \ref{fig:Gain3} shows that RGF is unaffected by the change in cost keeping PNE point fixed. However, with the increase in cost, PNE is shifted from \{S,S\} to \{S,N\} and thereby causing the drop in RGF. This implies fixing higher access price may not be beneficial for ISP under exogenous arrival of demand. 

%\section{Elastic Demand}
%In this section, we consider that the total demand is elastic and is dependent on subsidy factor.  That is, total demand is sensitive to change in subsidy offered by CPs. We model the total demand generated as $\tilde{\Lambda}=\Lambda+\Lambda_0(1-\gamma_1)+\Lambda_0(1-\gamma_1)$. We also continue to make Assumptions A1-A3. For convenience, we re-define $\overline{m}$ as $\overline{m}:=\sum_{i=1}^2 m_i -\tilde{\Lambda}=\sum_{i=1}^2 \tilde{m}_i -\Lambda$ where  $\tilde{m}_i=m_i-\Lambda_0(1-\gamma_i)$.The elastic traffic $\tilde\Lambda$ get splitted between CPs compettitively by the users based on the QoS experienced and the access price say $(\tilde\Lambda_1^*, \tilde\Lambda_2^*)$  which are set according to the Wardrop equilibrium as earlier as is given by
%\begin{equation}
%\tilde\Lambda_i^*=\Lambda_i+\Lambda_0(1-\gamma_i)=m_i-\frac{1}{\alpha-\gamma_i c} \forall i=1, 2
%\end{equation}
%
%where $\alpha:=\alpha(\gamma_1,\gamma_2)$ is the equilibrium cost given by
%\begin{equation}
%\alpha=\frac{c(\gamma_1+\gamma_2)}{2}+\frac{1}{\overline{m}}+ \sqrt{\frac{(c(\gamma_1-\gamma_2))^2}{4}+\frac{1}{\overline{m}^2}}.
%\end{equation}
%
%
%Similar to exogenous arrival model, we can define mean delay for end users and Utility of CPs. With these new definitions, all the results and properties obtained are similar to the exogenous arrival model. Infact, Non-cooperative game between CPs shows exactly same behaviour as that of exogenous model.


==> CPGame1_t.tex <==
In this section we assume that each CP either completely sponsor $(N)$ the access price or do not sponsor at all $(NS)$. The action profiles of the CPs can be then $(S,S), (N,N), (S,N),$ or $(N,S)$. Here, action profile $(S,N)$ indicates that $CP_1$ sponsors while $CP_2$ do not sponsor. For ease of notation we add subscripts $00, 11, 01, 10$ to the minimum equilibrium utility ($\alpha$) associated with each of these profiles. The following Theorem gives the equilibrium rates associated with these action profiles. 

\begin{thm}
	\label{thm:EquRatesSpecialCases}
	The equilibrium rates at different action profiles and the corresponding RGF are as follows:
	\begin{enumerate}
		\item For action profile $(S,S)$:
                     \\ $\tilde{\lambda_i^*}=m_i+\lambda_0-\frac{1}{\alpha_{00}} \;\; \forall i$  where $ \alpha_{00}=\frac{2}{\overline{m}}$ and  $RGF=1+\frac{2\lambda_0}{\lambda}$.
		\item For action profile $(N,N)$:
		\\$\tilde{\lambda_i^*}=m_i-\frac{1}{\alpha_{11}-c} \;\; \forall i$ where $\alpha_{11}=c+\frac{2}{\overline{m}}$ and  $RGF=1$, i.e., there is no revenue gain for ISP
		\item For action profile $(S,N)$:
		\\$\tilde{\lambda_1^*}=m_1+\lambda_0-\frac{1}{\alpha_{01}}$ and
		$\tilde{\lambda_2^*}=m_2-\frac{1}{\alpha_{01}-c}$ where $\alpha_{01}=c/2+1/\overline{m}+\sqrt{c^2/4+ 1/\overline{m}^2}$ and RGF is $1+\frac{\lambda_0}{\lambda}$
		\item For action profile $(N,S)$:
		\\$\tilde{\lambda_i^*}=m_1-\frac{1}{\alpha_{10}-c}$ and $\tilde{\lambda_2^*}=m_2+\lambda_0-\frac{1}{\alpha_{10}} $ where $\alpha_{10}=\alpha_{01}$ and $RGF=1+\frac{\lambda_0}{\lambda}.$%\hfill\IEEEQED
	\end{enumerate}
\end{thm}

\begin{cor}
	\label{corol:MinCostRelations}
	The minimum equilibrium costs satisfy the following properties
	\begin{itemize}
		\item $\alpha_{00}=\alpha_{11}-c$
		\item $\alpha_{01}\geq \alpha_{00}\geq \alpha_{10}-c$
		\item $c+ 1/\overline{m} \leq \alpha_{01}\leq c+ 2/\overline{m}$ 	\end{itemize}
\end{cor}

With each CP playing two actions $\{\textit{S,N}\}$ we have $2\times 2$ matrix games between the CPs. The utilities for both CPs over actions $\{\textit{S,N}\}$ are given in Table 1. 
%\begin{table}
%	\begin{center}
%		\begin{tabular}{|c|c|c|}\hline
%			$ A $ & $S $ & $ N $ \\ \hline
%			S & $U_1=(\beta-\rho c)(m_1-\lambda_0-1/\alpha_{00})$ & $U_1=(\beta-\rho c)(m_1-\lambda_0-1/\alpha_{01})%$ \\
%			$ $ & $U_2=(\beta-\rho c)(m_2-\lambda_0-1/\alpha_{00})$ & $U_2=\beta(m_2-\lambda_0-1/(\alpha_{01}-c))$ \%\ \hline
%			N & $U_1=\beta(m_1-\lambda_0-1/(\alpha_{10}-c))$ & $U_1=\beta(m_1-\lambda_0-1/(\alpha_{11}-c))$ \\
%			$ $ & $U_2=(\beta-\rho c)(m_2-\lambda_0-1/\alpha_{10})$ & $U_2=\beta(m_2-\lambda_0-1/(\alpha_{11}-c))$ \%\ \hline
%		\end{tabular}
%	\end{center}
%	\caption{Utility for CPs over actions $\{S,N\}$}  \label{tab:Utilities}
%\end{table}

\begin{table}
	\begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $S $ \\ \hline
			S & $U_1=(\beta-\rho c)(m_1+\lambda_0-1/\alpha_{00})$ \\
			$ $ & $U_2=(\beta-\rho c)(m_2+\lambda_0-1/\alpha_{00})$ \\ \hline
			N & $U_1=\beta(m_1+\lambda_0-1/(\alpha_{10}-c))$ \\
			$ $ & $U_2=(\beta-\rho c)(m_2+\lambda_0-1/\alpha_{10})$\\ \hline
		\end{tabular}
	\end{center}
    \begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ &$ N $ \\ \hline
			S & $U_1=(\beta-\rho c)(m_1+\lambda_0-1/\alpha_{01})$ \\
			$ $ & $U_2=\beta(m_2+\lambda_0-1/(\alpha_{01}-c))$ \\ \hline
			N & $U_1=\beta(m_1+\lambda_0-1/(\alpha_{11}-c))$ \\
			$ $ & $U_2=\beta(m_2+\lambda_0-1/(\alpha_{11}-c))$ \\ \hline
		\end{tabular}
	\end{center}
	\caption{Utility for CPs over actions $\{S,N\}$}  \label{tab:Utilities}
\end{table}

The following theorem states the conditions for the existence of PNE. 
\begin{thm}
	\label{thm:PNE}
Let $\rho, c, \beta$ be given. Then,
\begin{itemize}
	\item $(S,S)$ is a PNE if and only if  
	\begin{equation}
	\label{eqn:SS}
	\rho/\beta\leq A:=\frac{ 1/(\alpha_{10}-c)+\lambda_0-1/\alpha_{00}}{c(m_2+\lambda_0-1/\alpha_{00})}
	\end{equation}
	\item $(N,N)$ is a PNE if and only if 
	\begin{equation}
		\label{eqn:NN}
\rho/\beta \geq B:=\frac{1/(\alpha_{11}-c)+\lambda_0-1/\alpha_{01}}{c(m_1+\lambda_0-1/\alpha_{01})}
	\end{equation}
	\item $(S,N)$ is a PNE if and only if
	\begin{equation}
		\label{eqn:SN}
	\frac{ 1/(\alpha_{10}-c)+\lambda_0-1/\alpha_{00}}{c(m_2+\lambda_0-1/\alpha_{00})} \leq \rho/\beta \leq	\frac{1/(\alpha_{11}-c)+\lambda_0-1/\alpha_{01}}{c(m_1+\lambda_0-1/\alpha_{01})}
	\end{equation}
	\item $(N,S)$ is a PNE if and only if
	\begin{eqnarray}
		\label{eqn:NS}
C:=\frac{ 1/(\alpha_{10}-c)+\lambda_0-1/\alpha_{00}}{c(m_1+\lambda_0-1/\alpha_{00})} \leq \rho/\beta  \nonumber\\
\rho/\beta  \leq \frac{1/(\alpha_{11}-c)+\lambda_0-1/\alpha_{01}}{c(m_2+\lambda_0-1/\alpha_{01})}=:D.
	\end{eqnarray}
\end{itemize}
\end{thm}

\begin{cor}
	\label{corol:NoPNE}
	For all $c>0$, we have $C>D$ and hence $(N,S)$ cannot be a PNE.
\end{cor}
Theorem \ref{thm:PNE} gives a characterization of the PNE and figure \ref{fig:PNE1} depicts the range of $\rho/\beta$ for different PNE.

%\begin{figure*}[!h]
%	\centering
%		\subfloat[]{\includegraphics[scale=0.05]{figures/AB1}%
%		\label{fig:AB1}}
%	\hspace{0.6cm}
%	\subfloat[]{\includegraphics[scale=0.05]{figures/AB2}%
%		\label{fig:AB2}}
%		\caption {The comparision $A$ and $B$ with respect to change in parameters $c$ in Figs. \ref{fig:AB1} and \ref{fig:AB2} for different values of $m_1$.   We set $\beta=1$,$\rho=.9$, $\lambda=1200$, $\lambda_0=200$ and $m_2=1000$ throughout. In Fig. \ref{fig:AB1}, we set $m_1=900$ and in Fig. \ref{fig:AB2}, we set $m_1=650$.}
%	\label{fig:Gain}
%\end{figure*}

\begin{figure}[!h]
	\label{fig:PNE1}
	\centering
	\includegraphics[scale=.245]{figures/PNE1}
	\caption{The PNE as a function of $\rho/\beta$.}
\end{figure}

We study the behaviour of RGF and the shift in PNE point with respect to system parameters $\lambda,$ $\lambda_0$ and $c$ .  From Fig. \ref{fig:Gain1} it is observed that as $\lambda$ increases, RGF initially decreases steeply and then at a slower rate. This change is due to shift of PNE point from \{S,S\} to \{S,N\}. This shift of PNE point has been caused by the change in the values of A and B with the increase in $\lambda$. It is inferred that when CPS offer the subsidy, the gain for ISP decreases with increase in usual traffic flow, keeping exogenous traffic to be fixed.  Fig. \ref{fig:Gain2} shows that RGF initially increases at smaller rate with increase in exogenous traffic ($\lambda_0$) and later the rate increases. This shift in behaviour is again due to shifting PNE points from \{S,N\} to \{S,S\} as CPs are likely to go for full sponsorship if more exogenous traffic is generated. Thus, ISP is benefitted when higher exogenous traffic is generated as more revenue is generated. While Fig. \ref{fig:Gain3} shows that RGF is unaffected by the change in cost keeping PNE point fixed. However, with the increase in cost, PNE is shifted from \{S,S\} to \{S,N\} and thereby causing the drop in RGF. This implies fixing higher access price may not be beneficial for ISP under exogenous arrival of demand. 

\section{Elastic Demand}
In this section, we consider that the total demand is elastic and is dependent on subsidy factor.  That is, total demand is sensitive to change in subsidy offered by CPs. We model the total demand generated as $\tilde{\Lambda}=\Lambda+\Lambda_0(1-\gamma_1)+\Lambda_0(1-\gamma_1)$. We also continue to make Assumptions A1-A3. For convenience, we re-define $\overline{m}$ as $\overline{m}:=\sum_{i=1}^2 m_i -\tilde{\Lambda}=\sum_{i=1}^2 \tilde{m}_i -\Lambda$ where  $\tilde{m}_i=m_i-\Lambda_0(1-\gamma_i)$.The elastic traffic $\tilde\Lambda$ get splitted between CPs compettitively by the users based on the QoS experienced and the access price say $(\tilde\Lambda_1^*, \tilde\Lambda_2^*)$  which are set according to the Wardrop equilibrium as earlier as is given by
\begin{equation}
\tilde\Lambda_i^*=\Lambda_i+\Lambda_0(1-\gamma_i)=m_i-\frac{1}{\alpha-\gamma_i c} \forall i=1, 2
\end{equation}

where $\alpha:=\alpha(\gamma_1,\gamma_2)$ is the equilibrium cost given by
\begin{equation}
\alpha=\frac{c(\gamma_1+\gamma_2)}{2}+\frac{1}{\overline{m}}+ \sqrt{\frac{(c(\gamma_1-\gamma_2))^2}{4}+\frac{1}{\overline{m}^2}}.
\end{equation}


Similar to exogenous arrival model, we can define mean delay for end users and Utility of CPs. With these new definitions, all the results and properties obtained are similar to the exogenous arrival model. Infact, Non-cooperative game between CPs shows exactly same behaviour as that of exogenous model.


==> CPGame_t.tex <==
%% CP game with two actions.

%In this section we consider that  CPs only play either Sponsor (S) or Not-sponsor (N) actions, i.e., $\G_i \in \{0,1\} $ for all $i=1,2$ (no partial sponsorship is allowed). For ease of notation, we attach subscripts $00, 11, 01,$ and $10$ to the minimum equilibrium utility $\alpha$ to denote the cases where action of CPs are $(S,S), (N,N), (S,N),$ and $(N,S)$, respectively. The equilibrium rates for these actions profiles can be directly obtained from Lemma \ref{lma:EquRates}.
%
%\begin{thm}
%	\label{thm:EquRatesSpecialCases}
%	The equilibrium arrival rates when each CP either plays either S or N are as follows:
%	\begin{enumerate}
%		\item When actions are $(0,0)$:
%		$  \lambda_i^*=m_i-\frac{1}{\alpha_{00}} \;\; \mbox{for} \;\; i=1,2, \;\; \mbox{where} \;\; \alpha_{00}=\frac{2}{\overline{m}}$.
%		\item When the actions are $(1,1)$:
%		$\lambda_i^*=m_i-\frac{1}{\alpha_{11}-c} \;\; \mbox{for} \;\; i=1,2, \;\; \mbox{where} \;\; \alpha_{11}=c+\frac{2}{\overline{m}}$
%		\item When the actions are $(0,1)$:
%		$	\lambda_1^*=m_1-\frac{1}{\alpha_{01}} \;\;\mbox{and} \;\;
%		\lambda_2^*=m_2-\frac{1}{\alpha_{01}-c}$, where $\alpha_{01}=c/2+1/\overline{m}+\sqrt{c^2/4+ 1/\overline{m}^2}$. 
%		and can be bounded as
%		\begin{equation}
%		\label{eqn:DelayBounds}
%		c+ 1/\overline{m} \leq \alpha_{01}\leq c+ 2/\overline{m}.
%		\end{equation}
%		\item When the actions are $(1,0)$:
%		$\lambda_1^*=m_1-\frac{1}{\alpha_{10}-c} \;\;\mbox{and} \;\;
%		\lambda_2^*=m_2-\frac{1}{\alpha_{10}} 
%		\mbox{  where  } \alpha_{10}=\alpha_{01}$. %\hfill\IEEEQED
%	\end{enumerate}
%\end{thm}
%Note that under the action profile $(0,0)$ and $(1,1)$ the equilibrium arrival rates at the CPs remains the same, i.e., behavior of the users in the choice of CPs remains the same when both the CPs sponsor or both do not sponsor. When the CPs decisions are asymmetric, i.e., actions profile are $(1,0)$ or $(0,1)$, though the equilibrium arrival rates at the CPs are different, the minimum cost at equilibrium for the end users is the same. The relation between minimum equilibrium cost with different actions profiles is given as follows: 
%\begin{cor}
%	\label{corol:MinCostRelations}
%	We have $\alpha_{00}=\alpha_{11}-c$ and $\alpha_{01}\geq \alpha_{00}\geq \alpha_{10}-c$.
%\end{cor}
%
%With each CP playing two actions, we have a $2\times 2$ matrix game between the CPs which is guaranteed to have a mixed Nash equilibrium. We focus on existence of pure Nash equilibria (PNE) and derive conditions for their existence and analyze their properties. The utilities for both the CPs over actions $\{S, N\}$ are given in Table \ref{tab:Utilities}. 
%\begin{table}[H]
%	\begin{center}
%		\begin{tabular}{|c|c|c|}\hline
%			$ A $ & $S $ & $ N $ \\ \hline
%			S & $U_1=(\beta-\rho c)(m_1-1/\alpha_{00})$ & $U_1=(\beta-\rho c)(m_1-1/\alpha_{01})$ \\
%			$ $ & $U_2=(\beta-\rho c)(m_2-1/\alpha_{00})$ & $U_2=\beta(m_2-1/(\alpha_{01}-c))$ \\ \hline
%			N & $U_1=\beta(m_1-1/(\alpha_{10}-c))$ & $U_1=\beta(m_1-1/(\alpha_{11}-c))$ \\
%			$ $ & $U_2=(\beta-\rho c)(m_2-1/\alpha_{10})$ & $U_2=\beta(m_2-1/(\alpha_{11}-c))$ \\ \hline
%		\end{tabular}
%	\end{center}
%	\caption{Utility for CPs over actions $\{S,N\}$}  \label{tab:Utilities}
%\end{table}
%\noindent
%The following theorem states the conditions for the existence of PNE. 
%\begin{thm}
%	\label{thm:PNE}
%Let $\rho, c, \beta$ be given. Then,
%\begin{itemize}
%	\item $(S,S)$ is a PNE if and only if  
%	\begin{equation}
%	\label{eqn:SS}
%	\rho/\beta\leq A:=\frac{ 1/(\alpha_{10}-c)-1/\alpha_{00}}{c(m_2-1/\alpha_{00})}
%	\end{equation}
%	\item $(N,N)$ is a PNE if and only if 
%	\begin{equation}
%		\label{eqn:NN}
%\rho/\beta \geq B:=\frac{1/(\alpha_{11}-c)-1/\alpha_{01}}{c(m_1-1/\alpha_{01})}
%	\end{equation}
%	\item $(S,N)$ is a PNE if and only if
%	\begin{equation}
%		\label{eqn:SN}
%	\frac{ 1/(\alpha_{10}-c)-1/\alpha_{00}}{c(m_2-1/\alpha_{00})} \leq \rho/\beta \leq	\frac{1/(\alpha_{11}-c)-1/\alpha_{01}}{c(m_1-1/\alpha_{01})}
%	\end{equation}
%	\item $(N,S)$ is a PNE if and only if
%	\begin{eqnarray}
%		\label{eqn:NS}
%C:=\frac{ 1/(\alpha_{10}-c)-1/\alpha_{00}}{c(m_1-1/\alpha_{00})} \leq \rho/\beta  \nonumber\\
%\rho/\beta  \leq \frac{1/(\alpha_{11}-c)-1/\alpha_{01}}{c(m_2-1/\alpha_{01})}=:D.
%	\end{eqnarray}
%\end{itemize}
%\end{thm}
\begin{cor}
	\label{corol:NoPNE}
 For all $c>0$, we have $C>D$ and hence $(N,S)$ cannot be a PNE.
\end{cor}
As in the above corollary, it is easy to verify that $A\leq B$ for all $c$. Hence Theorem \ref{thm:PNE} gives a complete 
 characterization of the PNE. The following figure depicts the range of $\rho/\beta$ for different PNE profiles.
\begin{figure}[!h]
	\centering
	\includegraphics[scale=.4]{figures/PNE.pdf}
	\caption{The PNE as a function of $\rho/\beta$.}
\end{figure}



==> ExogenousArrivals1.tex <==
In the previous setup the total traffic rate is a constant and the total revenue for the ISP is $\lambda c$ irrespective of the subsidy set by the CPs. This makes the ISP indifferent to the differential pricing in the network. However, higher subsidy by the CPs may attract more traffic and in turn result in higher revenue for the ISP.  In fact, proponents of differential pricing argue that it encourages more people to access Internet content who otherwise coul not have afforded to do so because of high costs.  To account for this, we next consider a model with exogenous generation of traffic in addition to the usual traffic of rate $\lambda$. The exogenous traffic corresponds to the increased  demand that the CPs attract in addition to their usual traffic by offering subsidies which increases the total traffic generated by the users.  
Naturally, higher is the subsidy offered by an CP higher is the exogenous traffic it attracts. 
We model the exogenous traffic generated for $CP_i$ offering subsidy $\gamma_i$ to be linear in $\gamma_i$  and is given as $\lambda_0 (1-\gamma_i)$, where $\lambda_0 \geq 0 $ is a fixed constant. The total traffic for $CP_i, i=1,2$, when it attract the usual traffic $\lambda_i$ and offers subsidy $\gamma_i$ is then $\tilde{\lambda}_i=\lambda_i + \lambda_0 (1-\gamma_i)$, where $\lambda_1+\lambda_2 =\lambda$, and the total traffic in the networks is given by $\tilde{\lambda}:=\tilde{\lambda}(\gamma_1, \gamma_2)=\lambda + \sum_{i=1}^2 \lambda_0 (1-\gamma_i)$. For this case, the revenue generated by ISP is $\tilde{\lambda}c$ which increases if the CPs offer higher subsidy. To measure the gain in revenue for the ISP due to increased traffic from subsidies, we consider athe metric `Revenue Gain Factor' (RGF) defined as the ratio of ISP revenue under the non-neutral differential pricing scheme and that under the neutral regime where differential pricing is not allowed, i.e.,
\begin{multline}
RGF=\frac{(\lambda+\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2))\rho c}{\lambda \rho c} \\=1+\frac{\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2)}{\lambda}.
\end{multline}
We continue to make the assumptions $A1-A3$ as earlier. Note that with exogenous arrivals it may happen that $\sum_{i=1}^2 m_i < \tilde{\lambda}$ if the subsidy offered by the CPs is too high.


%we assume a model which 
%So far it has been assumed that demand arriving from users is constant and does not depend on the subsidy offered by content providers. Thereby, the total revenue generated by ISP is $\lambda c$, which is also independent of subsidy which makes ISP indifferent to subsidy rate as there is no incentive for him. However, in reality there may exist some exogenous demand which depends on the subsidy rate adding up to the total demand. In this section we consider the exogenous demand arrival to take into account the incentive for ISP.  The exogenous demand arrival for $i$th CP is assumed to be $\lambda_0(1-\gamma_i)$; $\lambda_0>=0$, implying higher the subsidy higher will be the exogenous demand arrival. Thus, new demand for $i$th CP is $\tilde{\lambda}_i=\lambda_i+\lambda_0(1-\gamma_i), \forall i=1,2,...,N$ and the total demand generated is give by $\tilde{\lambda}=\sum_{i=1}^N \tilde{\lambda_i}$.Under this case, the revenue generated by ISP is $(\lambda+\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2))c$. We define gain (incentive) for ISP as 
%\begin{multline}
%G=\frac{(\lambda+\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2))\rho c}{\lambda \rho c} \\=1+\frac{\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2)}{\lambda}
%\end{multline}

%Now, we will consider the game where there are only two CPs with exogenous demand arrival, with same set of assumptions as considered in previous model except the total capacity constraint. That is, the total capacity $\sum_{i=1}^ 2m_i$ is not necessarily less than that of new total demand, $\tilde{\lambda}$. For convenience, redefining $\overline{m}$ as $\overline{m}=\sum_{i=1}^2 m_i -\tilde{\lambda}=\sum_{i=1}^2 \tilde{m_i} -\lambda$ where  $\tilde{m_i}=m_i-\lambda_0(1-\gamma_i)$.

The usual traffic $\lambda$ gets split between the CPs competitively by the users based on the QoS experienced and the access price, whereas the exogenous traffic is fixed and depends only on the  subsidy factory. At equilibrium, the total traffic at $CP_i$ is given by $\tilde{\lambda}_i^*=\lambda_i^* + \lambda_0(1-\gamma_i)$ where $(\lambda_1^*, \lambda_2^*)$ are equilibrium flows set according to Wardrop criteria as earlier.


%where $\tilde{\lambda}_i^*=\lambda_i^* + \lambda_0(1-\gamma_i)$
With exogenous arrivals, mean delay defined in Section \ref{sec:MeanDelay} can be redefined as
\begin{equation}
D(c,\gamma_1,\gamma_2)=\sum_{i=1}^{N}\frac{\tilde{\lambda}_i^*}{\tilde{\lambda}}\frac{1}{m_i- \tilde{\lambda}_i^*}.
\end{equation}
%and the utility of $i$th CP is given as 
%\begin{equation}
%	U_i(\gamma_i, \gamma_{-i})=(\beta- (1-\gamma_i)\rho c)\tilde{\lambda}_i^*
%\end{equation}
The analysis of mean delay and the results derived in the previous sections remain the  same after replacing the capacities $m_1$ and $m_2$ by $m_1 -\lambda_0 (1-\gamma_1)$ and $m_2-\lambda_0(1-\gamma_2)$, respectively. 

We redefine the utilities of CPs with exogenous arrivals as 
\begin{equation}
\label{eqn:CPUtility_Exog}
U_i(\G_i, \G_{-i})=(\beta- (1-\G_i)\rho c)\tilde{\lambda}_i^* \quad \forall \; i=1,2.,
\end{equation}
With these new utilities, the condition for $CP_1$ to can earn higher revenue than that of $CP_2$ in Proposition \ref{prop:CP1larger} remains the same as in Proposition  \ref{prop:CP1larger} after replacing $\lambda$ by $\tilde{\lambda}$ and $\lambda_1^*$ by $\tilde{\lambda}_1^*$.
%
%\begin{proposition}
%Let $\overline{\beta}=\rho c/\beta\leq 1$. For a given $\gamma_2, \gamma_1\geq 0$, $U_1(\gamma_1,\gamma_2) \geq U_2(\gamma_2,\gamma_1)$ iff
%\begin{equation}
%\lambda_1^* \geq\frac{ \lambda+2\lambda_0-\lambda_0(\gamma_1+\gamma_2)}{\frac{1-(1-\gamma_1)\overline{\beta}}{1-(1-\gamma_2)\overline{\beta}}+1}-\lambda_0(1-\gamma_1).
%\end{equation}

%\end{proposition}
%Now, we analyze the utility function for the non cooperative game between the CPs for existence of Nash Equilibrium. 
Similar to previous model, the best response for CPs with exogenous traffic also have discontinuities and leads to non-existence of Nash equilibrium. We next focus our attention on the study of non cooperative game where CPs only play either Sponsor (S) or Not-sponsor (N) actions, i.e., $\G_i \in \{0,1\} $ for all $i=1,2$ (no partial sponsorship is allowed). 


\begin{figure*}[!h]
	\centering
		\subfloat[]{\includegraphics[scale=0.062]{figures/Gain1}%
		\label{fig:Gain1}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.39]{figures/Gain2}%
		\label{fig:Gain2}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.396]{figures/Gain3}%
		\label{fig:Gain3}}
	\caption {The change in gain for ISP and shift in PNE point is being studied with respect to change in parameters $\lambda$, $\lambda_0$ and $c$ in Figs. \ref{fig:Gain1}, \ref{fig:Gain2} and \ref{fig:Gain3} respectively.   We set $\beta=1$,$\rho=.9$, $m_1=700$ and $m_2=900$ throughout. In Fig. \ref{fig:Gain1}, we set $c=0.7$ and $\lambda_0=300$, in Fig. \ref{fig:Gain2}, we set $c=0.5$ and $\lambda=1000$ and in Fig. \ref{fig:Gain3}, we set $\lambda=100$ and $\lambda_0=300$.}
	\label{fig:Gain}
\end{figure*}


==> ExogenousArrivals_t.tex <==
In the previous setup the total traffic rate is a constant and the total revenue for the ISP is $\lambda c$ irrespective of the subsidy set by the CPs. This makes the ISP indifferent to the differential pricing in the network. However, higher subsidy by the CPs may attract more traffic and in turn result in higher revenue for the ISP. To account for this, we next consider a model with exogenous generation of traffic in addition to the usual traffic of rate $\lambda$. The exogenous traffic corresponds to the increased  demand that the CPs attract in addition to their usual traffic by offering subsidies which increases the total traffic generated by the users.  
Naturally, higher is the subsidy offered by an CP higher is the exogenous traffic it attracts. 
We model the exogenous traffic generated for $CP_i$ offering subsidy $\gamma_i$ to be linear in $\gamma_i$  and is given as $\lambda_0 (1-\gamma_i)$, where $\lambda_0 \geq 0 $ is a fixed constant. The total traffic for $CP_i, i=1,2$, when it attract the usual traffic $\lambda_i$ and offers subsidy $\gamma_i$ is then $\tilde{\lambda}_i=\lambda_i + \lambda_0 (1-\gamma_i)$, where $\lambda_1+\lambda_2 =\lambda$, and the total traffic in the networks is given by $\tilde{\lambda}:=\tilde{\lambda}(\gamma_1, \gamma_2)=\lambda + \sum_{i=1}^2 \lambda_0 (1-\gamma_i)$. For this case, the revenue generated by ISP is $\tilde{\lambda}c$ which increases if the CPs offer higher subsidy. To measure the gain in revenue for the ISP due to increased traffic from subsidies, we study the metric `Revenue Gain Factor' (RGF) defined as the ratio of ISP revenue under the non-neutral differential pricing scheme and that under the neutral regime where differential pricing is not allowed, i.e.,
\begin{multline}
RGF=\frac{(\lambda+\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2))\rho c}{\lambda \rho c} \\=1+\frac{\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2)}{\lambda}.
\end{multline}
We continue to make the assumptions $A1-A3$ as earlier. Note that with exogenous arrivals it may happen that $\sum_{i=1}^2 m_i < \tilde{\lambda}$ if the subsidy offered by the CPs is too high.


%we assume a model which 
%So far it has been assumed that demand arriving from users is constant and does not depend on the subsidy offered by content providers. Thereby, the total revenue generated by ISP is $\lambda c$, which is also independent of subsidy which makes ISP indifferent to subsidy rate as there is no incentive for him. However, in reality there may exist some exogenous demand which depends on the subsidy rate adding up to the total demand. In this section we consider the exogenous demand arrival to take into account the incentive for ISP.  The exogenous demand arrival for $i$th CP is assumed to be $\lambda_0(1-\gamma_i)$; $\lambda_0>=0$, implying higher the subsidy higher will be the exogenous demand arrival. Thus, new demand for $i$th CP is $\tilde{\lambda}_i=\lambda_i+\lambda_0(1-\gamma_i), \forall i=1,2,...,N$ and the total demand generated is give by $\tilde{\lambda}=\sum_{i=1}^N \tilde{\lambda_i}$.Under this case, the revenue generated by ISP is $(\lambda+\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2))c$. We define gain (incentive) for ISP as 
%\begin{multline}
%G=\frac{(\lambda+\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2))\rho c}{\lambda \rho c} \\=1+\frac{\lambda_0(1-\gamma_1)+\lambda_0(1-\gamma_2)}{\lambda}
%\end{multline}

%Now, we will consider the game where there are only two CPs with exogenous demand arrival, with same set of assumptions as considered in previous model except the total capacity constraint. That is, the total capacity $\sum_{i=1}^ 2m_i$ is not necessarily less than that of new total demand, $\tilde{\lambda}$. For convenience, redefining $\overline{m}$ as $\overline{m}=\sum_{i=1}^2 m_i -\tilde{\lambda}=\sum_{i=1}^2 \tilde{m_i} -\lambda$ where  $\tilde{m_i}=m_i-\lambda_0(1-\gamma_i)$.

The usual traffic $\lambda$ gets split between the CPs competitively by the users based on the QoS experienced and the access price, whereas the exogenous traffic is fixed and depends only on the  subsidy factory. At equilibrium, the total traffic at $CP_i$ is given by $\tilde{\lambda}_i^*=\lambda_i^* + \lambda_0(1-\gamma_i)$ where $(\lambda_1^*, \lambda_2^*)$ are equilibrium flows set according to Wardrop criteria as earlier.


%where $\tilde{\lambda}_i^*=\lambda_i^* + \lambda_0(1-\gamma_i)$
With exogenous arrivals, mean delay defined in Section \ref{sec:MeanDelay} can be redefined as
\begin{equation}
D(c,\gamma_1,\gamma_2)=\sum_{i=1}^{N}\frac{\tilde{\lambda}_i^*}{\tilde{\lambda}}\frac{1}{m_i- \tilde{\lambda}_i^*}.
\end{equation}
%and the utility of $i$th CP is given as 
%\begin{equation}
%	U_i(\gamma_i, \gamma_{-i})=(\beta- (1-\gamma_i)\rho c)\tilde{\lambda}_i^*
%\end{equation}
The analysis of mean delay and the results derived in the previous sections remain the  same after replacing the capacities $m_1$ and $m_2$ by $m_1 -\lambda_0 (1-\gamma_1)$ and $m_2-\lambda_0(1-\gamma_2)$, respectively, and $\sum_{i=1}^2 m_i \leq \tilde{\lambda}$.

The utilities of CPs with exogenous arrivals are
\begin{equation}
\label{eqn:CPUtility_Exog}
U_i(\G_i, \G_{-i})=(\beta- (1-\G_i)\rho c)\tilde{\lambda}_i^* \quad \forall \; i=1,2.
\end{equation}
With these new utilities, the condition for $CP_1$ to earn higher revenue than that of $CP_2$ remains the same as in Proposition  \ref{prop:CP1larger} after replacing $\lambda$ by $\tilde{\lambda}$ and $\lambda_1^*$ by $\tilde{\lambda}_1^*$, i.e., even with exogenous arrivals, the CP with lower QoS may earn higher revenue that that of the CP offering higher QoS.
%
%\begin{proposition}
%Let $\overline{\beta}=\rho c/\beta\leq 1$. For a given $\gamma_2, \gamma_1\geq 0$, $U_1(\gamma_1,\gamma_2) \geq U_2(\gamma_2,\gamma_1)$ iff
%\begin{equation}
%\lambda_1^* \geq\frac{ \lambda+2\lambda_0-\lambda_0(\gamma_1+\gamma_2)}{\frac{1-(1-\gamma_1)\overline{\beta}}{1-(1-\gamma_2)\overline{\beta}}+1}-\lambda_0(1-\gamma_1).
%\end{equation}
%\end{proposition}
%Now, we analyze the utility function for the non cooperative game between the CPs for existence of Nash Equilibrium. 
Similar to previous model, the best response for CPs with exogenous traffic also have discontinuities and leads to non-existence of Nash equilibrium. We next focus our attention on the study of non cooperative game where CPs only play either Sponsor (S) or Not-sponsor (N) actions, i.e., $\G_i \in \{0,1\} $ for all $i=1,2$ (no partial sponsorship is allowed). 


\begin{figure*}[!h]
	\centering
		\subfloat[]{\includegraphics[scale=0.062]{figures/Gain1}%
		\label{fig:Gain1}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.39]{figures/Gain2}%
		\label{fig:Gain2}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.396]{figures/Gain3}%
		\label{fig:Gain3}}
	\caption {The change in gain for ISP and shift in PNE point is being studied with respect to change in parameters $\lambda$, $\lambda_0$ and $c$ in Figs. \ref{fig:Gain1}, \ref{fig:Gain2} and \ref{fig:Gain3} respectively.   We set $\beta=1$,$\rho=.9$, $m_1=700$ and $m_2=900$ throughout. In Fig. \ref{fig:Gain1}, we set $c=0.7$ and $\lambda_0=300$, in Fig. \ref{fig:Gain2}, we set $c=0.5$ and $\lambda=1000$ and in Fig. \ref{fig:Gain3}, we set $\lambda=100$ and $\lambda_0=300$.}
	\label{fig:Gain}
\end{figure*}


==> MultiISPtmp.tex <==
In this section we extend our analysis for the case of oligopoly market with two ISPs. Each ISP connects both the CPs to the end users and set the access price independently. Knowing the access price,  the CPs set the subsidy factor for each ISP independently. Let $c_i, i=1,2$ denote the access price set by $ISP_i$  and $\gamma_j^i$ denote the subsidy factor set by $CP_j$ for traffic generated through $ISP_i$. We denote the traffic rate that flows to $CP_j$ from $ISP_i$ as $\lambda_j^i$. The exogenous traffic rate from $ISP_i$ to $CP_j$ is $\lambda_0(1-\lambda_j^i)$. 

\begin{figure}
	\centering
	\includegraphics[scale=.35]{figures/MultiISP}
	\caption{ Interaction between the Multi-ISP, CPs and end users.}
		\label{fig:Connections1}
\end{figure}


Therefore, the cost of an end user that connects via  $ISP_j$ to $CP_i$ while it is receiving traffic at rate $x$ is:
\begin{equation}
\label{eqn:MultiISPUserUtility}
C_i^j(x):=C_i^j(x,m_i,c_j,\gamma_j)=\begin{cases}
\frac{1}{m_i -x}  + \gamma_i^jc_j &\mbox{  if } m_i > x, \\
\infty &\mbox{otherwise.}
\end{cases}
\end{equation}

Let $\lambda_1^{*1},\lambda_1^{*2},\lambda_2^{*1},\lambda_2^{*2}$ denote the flows at equilibrium. 
\begin{lemma}
For $i,j=1,2$ $\lambda_{j}^{i*}>0$ iff $\gamma_j^*c_i < \gamma_j^*c_{-i}$ . 
\end{lemma} 
In order to compute the equilibrium, we have the following equalities:
\begin{eqnarray*}
\frac{1}{m_1-\lambda_1^1-\lambda_1^2}+\gamma_1^1c_1&=&\frac{1}{m_1-\lambda_1^1-\lambda_1^2}+\gamma_1^2c_2\\
&=&\frac{1}{m_2-\lambda_2^1-\lambda_2^2}+\gamma_2^1c_1\\
&=&\frac{1}{m_2-\lambda_2^1-\lambda_2^2}+\gamma_2^2c_2=\alpha
\end{eqnarray*}

with $\lambda_1^1+\lambda_1^2=\lambda_1 , \lambda_2^1+\lambda_2^2=\lambda_2$ and $ \lambda_1+\lambda_2=\lambda$. The set of eqautions can be solved to obtain equilibrium flows.

We assume that each CP can make an agreement with only one ISP and only full subsidizations are allowed, i.e. $\gamma_i^j \in \{0,1\}$. This decision is based on the traffic cost proposed by ISPs. The $CP_i$'s utility is:
$$
U_i(\gamma_i)=\sum_j(\beta_i^j-\rho(1-\gamma_i^j)c_j)\lambda_j^{i^*}.
$$ 
%We could consider the following assumptions:
%\begin{itemize}
%\item each CP can make an agreement with only one ISP,
%\item only fully subsidizations are allowed, i.e. $\gamma_i^j \in \{N,S\}$.
%\end{itemize}
Given these two constraints, the action set of each CP: $\{ SN, NS, NN\}$, where $SN$ denotes that CP sponsors $ISP_1$ and does not sponsor $ISP_2$.  
Finally, ISPs determine optimally this traffic cost factor maximizing their revenue:
$$
R_j(c)=\sum_{i}\lambda_j^{i*}c,
$$
where $\lambda_i^j$ is the equilibrium demand that depends on traffic cost and all the parameter of the model.

%Following gives the equilibrium arrival rates when each CP either plays SN, NS or NN:
%	\begin{enumerate}
%		\item When the actions are $(SN,SN)$:
%                    \\ $\lambda_1^{1*}=(m_1-\overline{m}/2), \lambda_1^{2*}=0, \lambda_2^{1*}=(m_2-\overline{m}/2)$ and $\lambda_2^{2*}=0$.
%		\item When the actions are $(SN,NS)$:
%		\\$\lambda_1^{1*}=(m_1-\overline{m}/2), \lambda_1^{2*}=0, \lambda_2^{1*}=0$ and $\lambda_2^{2*}=(m_2-\overline{m}/2)$.
%		\item When the actions are $ (SN,NN)$:
%		\\$\lambda_1^{1*}=m_1-1/\alpha, \lambda_1^{2*}=0, \lambda_2^{1*}=m_2-1/(\alpha-c_1
%)$ and $\lambda_2^{2*}=0$,
%\\where $\alpha=c_1/2+1/\overline{m}+\sqrt{c_1^2/4+ 1/\overline{m}^2}$
%		and can be bounded as $c_1+ 1/\overline{m} \leq \alpha\leq c_1+ 2/\overline{m}$.
%		
%		
%\item When the actions are $(NS,SN)$:
%		\\$\lambda_1^{1*}=0, \lambda_1^{2*}=(m_1-\overline{m}/2), \lambda_2^{1*}=(m_2-\overline{m}/2)$ and $\lambda_2^{2*}=0$.
%                     \item When the actions are $(NS,NS)$:
%		\\$\lambda_1^{1*}=0, \lambda_1^{2*}=(m_1-\overline{m}/2), \lambda_2^{1*}=0$ and $\lambda_2^{2*}=(m_2-\overline{m}/2)$.
%                     \item When the actions are $(NS,NN)$:
%		\\$\lambda_1^{1*}=0, \lambda_1^{2*}=m_1-1/\alpha, \lambda_2^{1*}=m_2-1/(\alpha-c_1)$ and $\lambda_2^{2*}=0$.
%
%                     \item When the actions are $(NN,SN)$:
%		\\$\lambda_1^{1*}=m_1-1/(\alpha-c_1), \lambda_1^{2*}=0, \lambda_2^{1*}=m_2-1/\alpha$ and $\lambda_2^{2*}=0$.
% 
%                     \item When the actions are $(NN,NS)$:
%		\\$\lambda_1^{1*}=m_1-1/(\alpha-c_1), \lambda_1^{2*}=0, \lambda_2^{1*}=0$ and $\lambda_2^{2*}=m_2-1/\alpha$
%            
%                     \item When the actions are $(NN,NN)$:
%		\\$\lambda_1^{1*}=(m_1-\overline{m}/2), \lambda_1^{2*}=0, \lambda_2^{1*}=(m_2-\overline{m}/2)$ and $\lambda_2^{2*}=0$.
%	\end{enumerate}
%


\begin{table}
	\begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $SN $ \\ \hline
			$SN$ & $U_1=(\beta_1^1-\rho c_1)(m_1-\overline{m}/2)$ \\
			$ $ & $U_2=(\beta_2^1-\rho c_1)(m_2-\overline{m}/2)$ \\ \hline
			$NS$ & $U_1=(\beta_1^2-\rho c_2)(m_1-\overline{m}/2)$ \\
			$ $ & $U_2=(\beta_2^1-\rho c_1)(m_2-\overline{m}/2)$\\ \hline
                                $NN$ & $U_1=\beta_1^1(m_1-1/(\alpha-c_1))$ \\
			$ $ & $U_2=(\beta_2^1-\rho c_1)(m_2-1/\alpha)$\\ \hline
		\end{tabular}
	\end{center}

           \begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $NS$ \\ \hline
			$SN$ & $U_1=(\beta_1^1-\rho c_1)(m_1-\overline{m}/2)$ \\
			$ $ & $U_2=(\beta_2^2-\rho c_2)(m_2-\overline{m}/2)$ \\ \hline
			$NS$ & $U_1=(\beta_1^2-\rho c_2)(m_1-\overline{m}/2)$ \\
			$ $ & $U_2=(\beta_2^2-\rho c_2)(m_2-\overline{m}/2)$\\ \hline
                                $NN$ & $U_1=\beta_1^1(m_1-1/(\alpha-c_1))$ \\
			$ $ & $U_2=(\beta_2^2-\rho c_2)(m_2-1/\alpha)$\\ \hline
		\end{tabular}
	\end{center}

           \begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $NN$ \\ \hline
			$SN$ & $U_1=(\beta_1^1-\rho c_1)(m_1-1/\alpha)$ \\
			$ $ & $U_2=\beta_2^1(m_2-1/(\alpha-c_1)$ \\ \hline
			$NS$ &  $U_1=(\beta_1^2-\rho c_2)(m_1-1/\alpha)$ \\
			$ $ & $U_2=\beta_2^1(m_2-1/(\alpha-c_1))$ \\ \hline
                                $NN$ & $U_1=\beta_1^1(m_1-\overline{m}/2)$ \\
			$ $ & $U_2=\beta_2^1(m_2-\overline{m}/2)$\\ \hline
		\end{tabular}
	\end{center}
	\caption{Utility for CPs over actions $\{SN,NS,NN\}$}  \label{tab:Utilities2}
\end{table}

\begin{thm}
	\label{thm:PNE2}
Let $\rho, c, \beta^i_j=\beta$ $\forall i,j$ be given. There are only four PNE: $(SN,SN)$, $(NN,NN)$  and $(SN,NN)$, and \begin{itemize}
	\item  $(SN, SN)$  is a PNE if and only if  
	\begin{equation}
	\label{eqn:SNSN}
	\rho/\beta \leq \frac{1/(\alpha-c_1)-\overline{m}/2}{c_1(m_2-\overline{m}/2)}
	\end{equation}
	\item  $(NN, NN)$ is a PNE if and only if 
	\begin{equation}
		\label{eqn:NNNN}
\rho/\beta \geq \frac{\overline{m}/2-1/\alpha}{c_1(m_1-1/\alpha)}
	\end{equation}
           \item $(SN, NN)$ is a PNE if and only if 
	\begin{equation}
		\label{eqn:SNNN}
\frac{1/(\alpha-c_1)-\overline{m}/2}{c_1(m_2-\overline{m}/2)}\leq \rho/\beta \leq \frac{\overline{m}/2-1/\alpha}{c_1(m_1-1/\alpha)} 
	\end{equation}
 %         \item $(NN, SN)$ is a PNE if and only if 
%	\begin{equation}
%		\label{eqn:31}
%\frac{1/(\alpha-c_1)-\overline{m}/2}{c_1(m_1-\overline{m}/2)}\leq \rho/\beta \leq \frac{\overline{m}/2-1/\alpha}{c_1(m_2-1/\alpha)} 
%	\end{equation}
\end{itemize}
\end{thm}



We now consider exogenous demand model and assume that the exogenous traffic generated for $CP_i$ offering subsidy $\gamma^j_i$ to $ISP_j$ is linear in $\gamma^ j_i$ and is given as $\lambda_0 (1-\gamma^ j_i)$, where $\lambda_0 \geq 0 $ is a fixed constant. The total traffic for $CP_i, i=1,2$ through $ISP_j, j=1, 2$, when it attract the usual traffic $\lambda^j_i$ and offers subsidy $\gamma^j_i$  is given by $\tilde{\lambda}^j_i =\lambda^j_i + \lambda_0 (1-\gamma^j_i)$. The total traffic generated for $CP_1$ is given by $\tilde{\lambda}_1:=\tilde{\lambda}_1(\gamma^1_1, \gamma^2_1)=\lambda_1 + \sum_{j=1}^2 \lambda_0 (1-\gamma^j_1)$, and for $CP_2$ is given by $\tilde{\lambda}_2:=\tilde{\lambda}_2(\gamma^1_2, \gamma^2_2)=\lambda_1 + \sum_{j=1}^2 \lambda_0 (1-\gamma^j_2)$. Thus, total traffic generated in the network is $\tilde{\lambda}=\tilde{\lambda}_1+\tilde{\lambda}_2$. For this case, the revenue generated by $ISP_j$ is $\sum_{i}\tilde{\lambda}_i^jc_j$ which increases if the CPs offer higher subsidy. The 'Revenue Gain Factor' (RGF) for each ISP is given as
\begin{multline}
RGF_1=\frac{(\lambda^1_1+\lambda^1_2+\lambda_0(1-\gamma^1_1)+\lambda_0(1-\gamma^1_2))\rho c_1}{(\lambda^1_1+\lambda^1_2) \rho c_1} \\=1+\frac{\lambda_0(1-\gamma^1_1)+\lambda_0(1-\gamma^1_2)}{\lambda^1_1+\lambda^1_2}
\end{multline}
\begin{multline}
RGF_2=\frac{(\lambda^2_1+\lambda^2_2+\lambda_0(1-\gamma^2_1)+\lambda_0(1-\gamma^2_2))\rho c_1}{(\lambda^2_1+\lambda^2_2) \rho c_1} \\=1+\frac{\lambda_0(1-\gamma^2_1)+\lambda_0(1-\gamma^2_2)}{\lambda^2_1+\lambda^2_2}
\end{multline}
 The $CP_i$'s utility is:
$$
U_i(\gamma_i)=\sum_j(\beta_i^j-\rho(1-\gamma_i^j)c_j)(\lambda_i^j+\lambda_0(1-\gamma_i^j)).
$$ 

The usual traffic $\lambda$ gets split between the CPs competitively by the users based on the QoS experienced and the access price, whereas the exogenous traffic is fixed and depends only on the subsidy factory. The total traffic at $CP_i$ is given by $\tilde{\lambda}^*_i=\sum_j \lambda_i^{j*}+\lambda_0 \sum_j(1-\gamma_i^j) $ where $\lambda_i^{j*} \forall i=1,2, j=1,2$ are set according to the Wardrop equilibrium as earlier.

\begin{table}
	\begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $SN $ \\ \hline
			$SN$ & $U_1=(\beta_1^1-\rho c_1)(m_1-\overline{m}/2+\lambda_0)$ \\
			$ $ & $U_2=(\beta_2^1-\rho c_1)(m_2-\overline{m}/2+\lambda_0)$ \\ \hline
			$NS$ & $U_1=(\beta_1^2-\rho c_2)(m_1-\overline{m}/2+\lambda_0)$ \\
			$ $ & $U_2=(\beta_2^1-\rho c_1)(m_2-\overline{m}/2+\lambda_0)$\\ \hline
                                $NN$ & $U_1=\beta_1^1(m_1-1/(\alpha-c_1))$ \\
			$ $ & $U_2=(\beta_2^1-\rho c_1)(m_2-1/\alpha+\lambda_0)$\\ \hline
		\end{tabular}
	\end{center}

           \begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $NS$ \\ \hline
			$SN$ & $U_1=(\beta_1^1-\rho c_1)(m_1-\overline{m}/2+\lambda_0)$ \\
			$ $ & $U_2=(\beta_2^2-\rho c_2)(m_2-\overline{m}/2+\lambda_0)$ \\ \hline
			$NS$ & $U_1=(\beta_1^2-\rho c_2)(m_1-\overline{m}/2+\lambda_0)$ \\
			$ $ & $U_2=(\beta_2^2-\rho c_2)(m_2-\overline{m}/2+\lambda_0)$\\ \hline
                                $NN$ & $U_1=\beta_1^1(m_1-1/(\alpha-c_1))$ \\
			$ $ & $U_2=(\beta_2^2-\rho c_2)(m_2-1/\alpha+\lambda_0)$\\ \hline
		\end{tabular}
	\end{center}

           \begin{center}
		\begin{tabular}{|c|c|c|}\hline
			$ A $ & $NN$ \\ \hline
			$SN$ & $U_1=(\beta_1^1-\rho c_1)(m_1-1/\alpha+\lambda_0)$ \\
			$ $ & $U_2=\beta_2^1(m_2-1/(\alpha-c_1))$ \\ \hline
			$NS$ &  $U_1=(\beta_1^2-\rho c_2)(m_1-1/\alpha+\lambda_0)$ \\
			$ $ & $U_2=\beta_2^1(m_2-1/(\alpha-c_1)$ \\ \hline
                                $NN$ & $U_1=\beta_1^1(m_1-\overline{m}/2)$ \\
			$ $ & $U_2=\beta_2^1(m_2-\overline{m}/2)$\\ \hline
		\end{tabular}
	\end{center}
	\caption{Utility for CPs over actions $\{SN,NS,NN\}$ in Exogenous case}  \label{tab:Utilities3}
\end{table}

\begin{figure*}[!h]
	\centering
		\subfloat[]{\includegraphics[scale=0.416]{figures/L1}%
		\label{fig:L1}}
	\hspace{0.0000cm}
	\subfloat[]{\includegraphics[scale=0.415]{figures/L0}%
		\label{fig:L0}}
	\hspace{0.00cm}
	\subfloat[]{\includegraphics[scale=0.439]{figures/c1}%
		\label{fig:c1}}
          	\hspace{0.00cm}
          	\subfloat[]{\includegraphics[scale=0.435]{figures/c2}%
		\label{fig:c2}}
	\caption {The change in gain for ISPs and shift in PNE point is being studied with respect to change in parameters $\lambda$, $\lambda_0$, $c_1$ and $c_2$in Figs. \ref{fig:L1}, \ref{fig:L0}, \ref{fig:c1} and \ref{fig:c2} respectively.We set $\beta=1$, $m_1=700$ and $m_2=900$ throughout. In Fig. \ref{fig:L1}, we set $c_1=0.7$, $c_2=0.9$, $\rho=0.9$ and $\lambda_0=300$, in Fig. \ref{fig:L0}, we set $c_1=0.7$, $c_2=0.9$, $\rho=0.9$ and $\lambda=900$, in Fig. \ref{fig:c1}, we set $c_2=0.9$, $\rho=0.8$ $\lambda=1000$ and $\lambda_0=300$ and  in Fig. \ref{fig:c2}, we set $c_1=0.4$, $\rho=0.9$ $\lambda=1200$ and $\lambda_0=250$.}
	\label{fig:RGF2}
\end{figure*}

Following give equillirbrium arrival rates anda RGF when each CP either plays SN, NS or NN. 

	\begin{enumerate}
		\item When the actions are $(SN,SN)$:
                    \\ $\lambda_1^{1*}=(m_1-\overline{m}/2+\lambda_0), \lambda_1^{2*}=0, \lambda_2^{1*}=(m_2-\overline{m}/2+\lambda_0)$ and $\lambda_2^{2*}=0$.
\\$RGF_1=1+\frac{2\lambda_0}{\lambda}$ and $RGF_2=1$.
		
                     \item When the actions are $(SN,NS)$:
		\\$\lambda_1^{1*}=(m_1-\overline{m}/2+\lambda_0), \lambda_1^{2*}=0, \lambda_2^{1*}=0$ and $\lambda_2^{2*}=(m_2-\overline{m}/2+\lambda_0)$.
                \\$RGF_1=1+\frac{\lambda_0}{\lambda_1^{1*}}$ and $RGF_2=1+\frac{\lambda_0}{\lambda_2^{2*}}$.
		
                     \item When the actions are $ (SN,NN)$:
		\\$\lambda_1^{1*}=m_1-1/\alpha+\lambda_0, \lambda_1^{2*}=0, \lambda_2^{1*}=m_2-1/(\alpha-c_1
)$ and $\lambda_2^{2*}=0$, where $\alpha=c_1/2+1/\overline{m}+\sqrt{c_1^2/4+ 1/\overline{m}^2}$
		and can be bounded as $c_1+ 1/\overline{m} \leq \alpha\leq c_1+ 2/\overline{m}$.
		\\$RGF_1=1+\frac{\lambda_0}{\lambda}$ and $RGF_2=1$.
		
                    \item When the actions are $(NS,SN)$:
		\\$\lambda_1^{1*}=0, \lambda_1^{2*}=(m_1-\overline{m}/2+\lambda_0), \lambda_2^{1*}=(m_2-\overline{m}/2+\lambda_0)$ and $\lambda_2^{2*}=0$.
                   \\$RGF_1=1+\frac{\lambda_0}{\lambda_2^{1*}}$ and $RGF_2=1+\frac{\lambda_0}{\lambda_2^{2*}}$.

                     \item When the actions are $(NS,NS)$:
		\\$\lambda_1^{1*}=0, \lambda_1^{2*}=(m_1-\overline{m}/2+\lambda_0), \lambda_2^{1*}=0$ and $\lambda_2^{2*}=(m_2-\overline{m}/2+\lambda_0)$.
                      \\$RGF_1=1$ and $RGF_2=1+\frac{2\lambda_0}{\lambda}$.

                     \item When the actions are $(NS,NN)$:
		\\$\lambda_1^{1*}=0, \lambda_1^{2*}=m_1-1/\alpha+\lambda_0, \lambda_2^{1*}=m_2-1/(\alpha-c_1)$ and $\lambda_2^{2*}=0$.
                     \\$RGF_1=1$ and $RGF_2=1+\frac{\lambda_0}{\lambda_2^{1*}}$.

                     \item When the actions are $(NN,SN)$:
		\\$\lambda_1^{1*}=m_1-1/(\alpha-c_1), \lambda_1^{2*}=0, \lambda_2^{1*}=m_2-1/\alpha+\lambda_0$ and $\lambda_2^{2*}=0$.
                \\$RGF_1=1+\frac{\lambda_0}{\lambda}$ and $RGF_2=1$.
 
                     \item When the actions are $(NN,NS)$:
		\\$\lambda_1^{1*}=m_1-1/(\alpha-c_1), \lambda_1^{2*}=0, \lambda_2^{1*}=0$ and $\lambda_2^{2*}=m_2-1/\alpha+\lambda_0$
                \\$RGF_1=1$ and $RGF_2=1+\frac{\lambda_0}{\lambda_2^{2*}}$.
           
                     \item When the actions are $(NN,NN)$:
		\\$\lambda_1^{1*}=(m_1-\overline{m}/2), \lambda_1^{2*}=0, \lambda_2^{1*}=(m_2-\overline{m}/2)$ and $\lambda_2^{2*}=0$.
                \\$RGF_1=1$ and $RGF_2=1$. 

	\end{enumerate}

Foloowing theorem gives characterization of PNE.

\begin{thm}
	\label{thm:PNE2}
Let $\rho, c, \beta^i_j=\beta$ $\forall i,j$ be given. There are only three PNE: $(SN,SN)$, $(NN,NN)$, and $(SN,NN)$, and 
\item  $(SN, SN)$  is a PNE if and only if  
	\begin{equation}
	\label{eqn:SNSN}
	\rho/\beta \leq \frac{1/(\alpha-c_1)-\overline{m}/2+\lambda_0}{c_1(m_2-\overline{m}/2+\lambda_0)}
	\end{equation}

	\item  $(NN, NN)$ is a PNE if and only if 
	\begin{equation}
		\label{eqn:NNNN}
\rho/\beta \geq \frac{\overline{m}/2-1/\alpha+\lambda_0}{c_1(m_1-1/\alpha+\lambda_0)}
	\end{equation}
          
 \item $(SN, NN)$ is a PNE if and only if 
	\begin{equation}
		\label{eqn:31}
\frac{1/(\alpha-c_1)-\overline{m}/2+\lambda_0}{c_1(m_2-\overline{m}/2+\lambda_0)}\leq \rho/\beta \leq \frac{\overline{m}/2-1/\alpha+\lambda_0}{c_1(m_1-1/\alpha+\lambda_0)} 
	\end{equation}
\end{thm}

We study the behaviour of RGF at different PNE points and the shift in PNE point with respect to system parameters $\lambda,$ $\lambda_0$ and $c_1$ and $c_2$. Since at PNE, none of the CPs makes sponsorship with $ISP_2$ (ISP with higher access price), RGF of $ISP_2$ remain same. Therefore, we focus on the revenue gain of $ISP_1$. It can be seen from Figs. \ref{fig:L1}-\ref{fig:c1} that the behaviour of RGF of $ISP_1$ is exactly same as that of single ISP case. And there is no affect of $c_2$ on RGF for both ISPs which is because $c_2>c_1$ and have no affect on PNE points.  


% From Fig. \ref{fig:L1} it is observed that as $\lambda$ increases, RGF decreases and PNE point for CPs get shifted from\{SN,SN\} to \{NN,NS\}. It is inferred that when intrinsic traffic is low both CPs will sponsor to attract more traffic and with higher intrinsic traffic only CP with higher capacity will sponsor. Fig. \ref{fig:L0} shows that RGF initially increases with increase in exogenous traffic ($\lambda_0$) and PNE point get shifted from \{SN,SN\} to \{NN,NS\}.  That is, when endogenous traffic is low both CPs will sponsor to attract more traffic, however, as endogenous traffic increases only CP with higher capacity will sponsor. ISP is also benefitted when higher exogenous traffic is generated. Fig. \ref{fig:c1} shows that as the access price set by $ISP_1$ increases, RGF decreases as PNE point get shifted from \{NN,NS\} to \{NN,NN\}. That is, at higher access price none of the CPs will sponsor and ISP doesn’t get any benefit by setting high access price. While Fig. \ref{fig:c2} shows that as the access price set by $ISP_2$ increases, RGF increases as PNE point get shifted from \{NN,NN\} to \{NN,NS\}. That is, CP will sponsor with ISP with lower access price as the ISP with higher access price increases its cost. This also implies ISP doesn’t get any benefit by setting high access price. That is, there is indirect price war between ISPs and by setting lower access price, they get more benefit. 

